Saying Hello World with GrGen.NET - A Solution to the TTC 2011 Instructive Case

We introduce the graph transformation tool GrGen.NET (www.grgen.net) by solving the Hello World Case of the Transformation Tool Contest 2011 which consists of a collection of small transformation tasks; for each task a section is given explaining our implementation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{281}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.23}{10.4204/EPTCS.74.23}}
\pdfoutput=1

